Statistical physics and approximate message-passing algorithms for sparse linear estimation problems in signal processing and coding theory

This thesis is interested in the application of statistical physics methods and inference to sparse linear estimation problems. The main tools are the graphical models and approximate message-passing algorithm together with the cavity method. We will also use the replica method of statistical physics of disordered systems which allows to associate to the studied problems a cost function referred as the potential of free entropy in physics. It allows to predict the different phases of typical complexity of the problem as a function of external parameters such as the noise level or the number of measurements one has about the signal: the inference can be typically easy, hard or impossible. We will see that the hard phase corresponds to a regime of coexistence of the actual solution together with another unwanted solution of the message passing equations. In this phase, it represents a metastable state which is not the true equilibrium solution. This phenomenon can be linked to supercooled water blocked in the liquid state below its freezing critical temperature. We will use a method that allows to overcome the metastability mimicing the strategy adopted by nature itself for supercooled water: the nucleation and spatial coupling. In supercooled water, a weak localized perturbation is enough to create a crystal nucleus that will propagate in all the medium thanks to the physical couplings between closeby atoms. The same process will help the algorithm to find the signal, thanks to the introduction of a nucleus containing local information about the signal. It will then spread as a "reconstruction wave" similar to the crystal in the water. After an introduction to statistical inference and sparse linear estimation, we will introduce the necessary tools. Then we will move to applications of these notions to signal processing and coding theory problems.

==> head/abstracts.tex <==
%\begingroup
%\let\cleardoublepage\clearpage


% English abstract
% \cleardoublepage
\chapter*{Abstract}
%\markboth{Abstract}{Abstract}
\addcontentsline{toc}{chapter}{Abstract (English/Français)} % adds an entry to the table of contents
This thesis is interested in the application of statistical physics methods and inference to signal processing and coding theory, more precisely, to sparse linear estimation problems.
\vskip0.2cm

The main tools are essentially the graphical models and the approximate message-passing algorithm together with the cavity method (referred as the state evolution analysis in the signal processing context) for its theoretical analysis. We will also use the replica method of statistical physics of disordered systems which allows to associate to the studied problems a cost function referred as the potential of free entropy in physics. It allows to predict the different phases of typical complexity of the problem as a function of external parameters such as the noise level or the number of measurements one has about the signal: the inference can be typically easy, hard or impossible. We will see that the hard phase corresponds to a regime of coexistence of the actual solution together with another unwanted solution of the message passing equations. In this phase, it represents a metastable state which is not the true equilibrium solution. This phenomenon can be linked to supercooled water blocked in the liquid state below its freezing critical temperature.
\vskip0.2cm

Thanks to this understanding of blocking phenomenon of the algorithm, we will use a method that allows to overcome the metastability mimicing the strategy adopted by nature itself for supercooled water: the nucleation and spatial coupling. In supercooled water, a weak localized perturbation is enough to create a crystal nucleus that will propagate in all the medium thanks to the physical couplings between closeby atoms. The same process will help the algorithm to find the signal, thanks to the introduction of a nucleus containing local information about the signal. It will then spread
as a "reconstruction wave" similar to the crystal in the water.
\vskip0.2cm

After an introduction to statistical inference and sparse linear estimation, we will introduce the necessary tools. Then we will move to applications of these notions. They will be divided into two parts.
\vskip0.2cm

The signal processing part will focus essentially on the compressed sensing problem
where we seek to infer a sparse signal from a small number of linear projections of it that can be noisy. We will study in details the influence of structured operators instead of purely random ones used originally in compressed sensing. These allow a substantial gain in computational complexity and necessary memory allocation, which are necessary conditions in order to work with very large signals. We will see that the combined use of such operators with spatial coupling allows the implementation of an highly optimized algorithm able to reach near to optimal performances. We will also study the algorithm behavior for reconstruction of approximately sparse signals, a fundamental question for the application of compressed sensing to real life problems. A direct application will be studied via the reconstruction of images measured by fluorescence microscopy. The reconstruction of "natural" images will be considered as well. 
\vskip0.2cm

In coding theory, we will look at the message-passing decoding performances for two distincts real noisy channel models. A first scheme where the signal to infer will be the noise itself will be presented. The second one, the sparse superposition codes for the additive white Gaussian noise channel is the first example of error correction scheme directly interpreted as a structured compressed sensing problem. Here we will apply all the tools developed in this thesis for finally obtaining a very promising decoder that allows to decode at very high transmission rates, very close of the fundamental channel limit.

\vskip0.5cm
\textbf{Keywords:} Statistical physics, disordered systems, mean field theory, signal processing, Bayesian inference, statistical learning, coding theory, linear estimation, sparsity, approximate sparsity, compressed sensing, spatial coupling, Gaussian channel, error correcting codes, sparse superposition codes, approximate message passing algorithm, cavity method, state evolution analysis, replica method.
%
%
%
% French abstract
\begin{otherlanguage}{french}
\cleardoublepage
\chapter*{Résumé}
%
Cette thèse s'intéresse à l'application de méthodes de physique statistique des systèmes désordonnés ainsi que de l'inférence à des problèmes issus du traitement du signal et de la théorie du codage, plus précisément, aux problèmes parcimonieux d'estimation linéaire.
\vskip0.2cm

Les outils utilisés sont essentiellement les modèles graphiques et l'algorithme approximé de passage de messages ainsi que la méthode de la cavité (appelée analyse de l'évolution d'état dans le contexte du traitement de signal) pour son analyse théorique. Nous aurons également recours à la méthode des répliques de la physique des systèmes désordonnées qui permet d'associer aux problèmes rencontrés une fonction de coût appelé potentiel ou entropie libre en physique. Celle-ci permettra de prédire les différentes phases de complexité typique du problème, en fonction de paramètres externes tels que le niveau de bruit ou le nombre de mesures liées au signal auquel l'on a accès: l'inférence pourra être ainsi typiquement simple, possible mais difficile et enfin impossible. Nous verrons que la phase difficile correspond à un régime où coexistent la solution recherchée ainsi qu'une autre solution des équations de passage de messages. Dans cette phase, celle-ci est un état métastable et ne représente donc pas l'équilibre thermodynamique. Ce phénomène peut-être rapproché de la surfusion de l'eau, bloquée dans l'état liquide à une température où elle devrait être solide pour être à l'équilibre. 
\vskip0.2cm

Via cette compréhension du phénomène de blocage de l'algorithme, nous utiliserons une méthode permettant de franchir l'état métastable en imitant la stratégie adoptée par la nature pour la surfusion: la nucléation et le couplage spatial. Dans de l'eau en état métastable liquide, il suffit d'une légère perturbation localisée pour que se créer un noyau de cristal qui va rapidement se propager dans tout le système de proche en proche grâce aux couplages physiques entre atomes. Le même procédé sera utilisé pour aider l'algorithme à retrouver le signal, et ce grâce à l'introduction d'un noyau contenant de l'information locale sur le signal. Celui-ci se propagera ensuite via une "onde de reconstruction" similaire à la propagation de proche en proche du cristal dans l'eau.
\vskip0.2cm

Après une introduction à l'inférence statistique et aux problèmes d'estimation linéaires, on introduira les outils nécessaires. Seront ensuite présentées des applications de ces notions. Celles-ci seront divisées en deux parties.
\vskip0.2cm

La partie traitement du signal se concentre essentiellement sur le problème de l'acquisition comprimée où l'on cherche à inférer un signal parcimonieux dont on connaît un nombre restreint de projections linéaires qui peuvent être bruitées. Est étudiée en profondeur l'influence de l'utilisation d'opérateurs structurés à la place des matrices aléatoires utilisées originellement en acquisition comprimée. Ceux-ci permettent un gain substantiel en temps de traitement et en allocation de mémoire, conditions nécessaires pour le traitement algorithmique de très grands signaux. Nous verrons que l'utilisation combinée de tels opérateurs avec la méthode du couplage spatial permet d'obtenir un algorithme de reconstruction extrêmement optimisé et s'approchant des performances optimales. Nous étudierons également le comportement de l'algorithme confronté à des signaux seulement approximativement parcimonieux, question fondamentale pour l'application concrète de l'acquisition comprimée sur des signaux physiques réels. Une application directe sera étudiée au travers de la reconstruction d'images mesurées par microscopie à fluorescence. La reconstruction d'images dites "naturelles" sera également étudiée. 
\vskip0.2cm

En théorie du codage, seront étudiées les performances du décodeur basé sur le passage de message pour deux modèles distincts de canaux continus. Nous étudierons un schéma où le signal inféré sera en fait le bruit que l'on pourra ainsi soustraire au signal reçu. Le second, les codes de superposition parcimonieuse pour le canal additif Gaussien est le premier exemple de schéma de codes correcteurs d'erreurs pouvant être directement interprété comme un problème d'acquisition comprimée structuré. Dans ce schéma, nous appliquerons une grande partie des techniques étudiée dans cette thèse pour finalement obtenir un décodeur ayant des résultats très prometteurs à des taux d'information transmise extrêmement proches de la limite théorique de transmission du canal.

\vskip0.5cm
\textbf{Mots clefs:} Physique statistique, systèmes  désordonnés, théorie du champ moyen, traitement du signal, inférence Bayesienne, apprentissage statistique, théorie du codage, estimation linéaire, parcimonie, parcimonie approximative, acquisition comprimée, couplage spatial, canal Gaussien, codes correcteurs d'erreurs, codes de superposition parcimonieuse, algorithme approximé de passage de messages, méthode de la cavité, analyse d'évolution des états, méthode des répliques.
\end{otherlanguage}


%\endgroup			
%\vfill

==> head/acknowledgements.tex <==
\cleardoublepage
\chapter*{Remerciements}
\markboth{Remerciements}{Remerciements}
\addcontentsline{toc}{chapter}{Remerciements}

Je tiens avant tout à remercier mes parents qui m’ont toujours laissé totalement libre de mes choix et m’ont tout donné, qui m’ont soutenu pendant cette longue période souvent difficile, parfois très difficile et toujours merveilleuse qu’ont été mes études. Merci à mes soeurs, Louise et Virginie. Merci à toute ma famille, présente dans les joies et difficultés.

Je remercie mon directeur Florent, le maitre Jedi, un ami. Merci de m’avoir fait confiance, de m’avoir enseigné par la pratique le vrai sens critique, de m’avoir présenté tant de personnes incroyables, de m’avoir offert ces expériences enrichissantes en école et ailleurs, d’avoir été insupportable quand il le fallait vraiment et d’avoir toujours su trouver l’équilibre entre pression et liberté, travail et humour, entre aide et indépendance. Je n’aurais réellement pas pu vivre une meilleure expérience pour mon doctorat.

Merci à Eric Tramel et Francesco Caltagirone pour leur sympathie et leurs explications.

Je tiens à remercier ceux qui ont rendu ma thèse encore plus agréable par leur amitié, qui ont transformé tous mes repas (et soirées) en moments toujours plus marrants, qui m’ont presentés leurs amis... Merci Thim, Thomas, le petit Christophe, Alaa, Alice, Antoine, Sophie, Ralph et merci à tous les autres aussi.

Je voudrais également remercier ceux qui m'ont permis d'en arriver là. En particulier Riccardo Zecchina qui m'a fait découvrir les domaines de l'inférence et de la belle physique statistique du désordre, Alessandro Pelizzola qui a tout fait pour rendre mon année à Turin si enrichissante et simple, Silvio Franz et Emmanuel Trizac pour m'avoir fait confiance en m'envoyant en Italie, merci à Marc Mézard pour son influence directe ou indirecte dans tous les travaux auxquels j'ai pu m'intéresser pendant ces trois années et demie, sur tous les papiers que j'ai pu lire et pour m'avoir montré ce que c'est que de vraiment savoir skier... Merci à Lenka Zdeborova pour ces collaborations fructueuses, Laurent Daudet pour m'avoir aidé à prendre des décisions importantes. 

Merci aussi à Rüdiger Urbanke et Nicolas Macris pour leur accueil à Lausanne. J'attends avec impatience les années à venir... Merci aux autres membres de mon jury de prendre le temps pour ma soutenance et avoir la patience de lire ma thèse: David Saad, Federico Ricci-Tersenghi et Marc Lelarge.

Je n’oublie pas les membres de mon premier lieu de travail, le laboratoire de physico-chimie théorique de l’École Supérieure de physique et chimie de Paris, en particulier Élie Raphaël et Thomas Salez pour leur sympathie perpétuelle, ainsi que Justine et Antoine.

Je dois beaucoup à mes colocataires qui m’auront supporté malgré mes crises de nerfs suite à trop de message-passing et avec qui j’aurais tellement rigolé: Charlotte, PH et Manon, vous êtes les meilleurs.

Merci Auré d'avoir rendu mes études encore plus intéressantes, du début à la fin. 

Je n'oublie pas Brian et tous les serveurs de Chez Léa sans qui cette période de rédaction aurait été très différente...

Je tiens également à remercier la DGA de m'avoir financé.

La liste pourrait encore continuer longtemps ayant rencontré tellement de gens intéressants et sympathiques durant ces années, merci à vous tous..

\bigskip
 
\noindent\textit{Paris, 20 Mai 2015}
\hfill J.~B.

==> head/dedication.tex <==
\cleardoublepage
\thispagestyle{empty}


\vspace*{3cm}

\begin{raggedleft}
    	La science c'est plutôt cool quand même...\\    		
\end{raggedleft}

\vspace{4cm}

\begin{center}
    A mes parents qui m'ont tout donné et mes soeurs que j'aime par dessus tout.\\
    Merci de m'avoir supporté jusqu'ici...
\end{center}

==> head/settings_custom.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%		Thesis Settings
%		Custom settings
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{cite}
\usepackage{array}
\usepackage{url}
\usepackage[utf8]{inputenc}  
% \usepackage{citesort}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{algpseudocode} 
\usepackage{marginnote}
\usepackage{rotating}
\usepackage{float}

\setcounter{page}{1}

\bibliographystyle{IEEEtran}

% new commands
\newcommand*\NewPage{\null\thispagestyle{empty}\newpage}
\DeclareUnicodeCharacter{00A0}{~}
\def \L{{\cal L}}
\def \({\left(}
\def \){\right)}
\def \[{\left[}
\def \]{\right]}
\newcommand{\tbf}[1]{{\textbf{#1}}}
\newcommand{\bsy}[1]{{\boldsymbol{#1}}}
\newcommand{\txt}[1]{\text{#1}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\cv}[1]{\underline{#1}}
\newcommand{\bQ}{{\textbf {Q}}}
\newcommand{\bq}{{\textbf {q}}}
\newcommand{\bm}{{\textbf {m}}}
\newcommand{\br}{{\textbf {r}}}
\newcommand{\bF}{{\textbf {F}}}
\newcommand{\bff}{{\textbf {f}}}
\newcommand{\bG}{{\textbf {G}}}
\newcommand{\bW}{{\textbf {W}}}
\newcommand{\bh}{{\textbf {h}}}
\newcommand{\bw}{{\textbf {w}}}
\newcommand{\bv}{{\textbf {v}}}
\newcommand{\bA}{{\textbf {A}}}
\newcommand{\bB}{{\textbf {B}}}
\newcommand{\bhx}{\hat {\textbf {x}}}
\newcommand{\bX}{{\textbf {X}}}
\newcommand{\bx}{{\textbf {x}}}
\newcommand{\bo}{{\textbf {o}}}
\newcommand{\blambda}{{\boldsymbol{\Lambda}}}
\newcommand{\btau}{{\boldsymbol{\tau}}}
\newcommand{\by}{{\textbf {y}}}
\newcommand{\bz}{{\textbf {z}}}
\newcommand{\bl}{{\textbf {l}}}
\newcommand{\bs}{{\textbf {s}}}
\newcommand{\bS}{{\textbf {S}}}
\newcommand{\bc}{{\textbf {c}}}
\newcommand{\bk}{{\textbf {k}}}
\newcommand{\bR}{{\textbf {R}}}
\newcommand{\beps}{{\boldsymbol {\epsilon}}}
\newcommand{\bxigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bxi}{{\boldsymbol{\xi}}}
\newcommand{\bzero}{{\textbf{0}}}
\newcommand{\ba}{{\textbf {a}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\lab}[1]{\label{#1}}
\newcommand{\bxii}{{\boldsymbol{\xi}}}
\newcommand{\bre}{{\textbf {e}}}
\newcommand{\bytilde}{{\tilde{\textbf {y}}}}
\newcommand{\bxhat}{{\tilde{\textbf {x}}}}
\newcommand{\mc}{\mathcal}
\newcommand{\eps}{\varepsilon}
\newcommand{\calF}{\mathcal F}
\newcommand{\s}{\sigma}
\renewcommand{\d}{\text{d}}
\newcommand{\e}{\text {e}}
\newcommand{\ds}{\Delta\sigma}
\newcommand{\hw}{h^{\rm W}}
\newcommand{\sw}{\sigma^{\rm W}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\de}{\partial}
\newcommand{\eq}{\text{ eq}}
\newcommand{\sign}{\text{ sign}}
\newcommand{\ua}{\uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\mE}{\mathbb{E}}

==> head/structure.tex <==
\cleardoublepage
\chapter*{Structure of the thesis}


==> head/titlepage.tex <==
\begin{titlepage}
\begin{center}
% \large
\sffamily


\null\vspace{2cm}
{\LARGE STATISTICAL PHYSICS AND\\[3pt]APPROXIMATE MESSAGE PASSING ALGORITHMS\\[3pt]FOR SPARSE LINEAR ESTIMATION PROBLEMS\\[12pt]IN SIGNAL PROCESSING AND CODING THEORY}
    
\vfill

\begin{tabular} {cc}
\parbox{0.3\textwidth}{\includegraphics[width=2.65cm]{./images/LogoENS.png}\\[6pt]
					   \includegraphics[width=2.65cm]{./images/LogoP7.png}}
&
\parbox{0.7\textwidth}{%
	Thèse n. \\
	présentée le 18 septembre 2015\\
	à l'\'Ecole Normale Supérieure de Paris.\\
	Travail effectué au laboratoire de physique statistique\\
	de l'\'Ecole Normale Supérieure de Paris\\
	sous la direction de Prof. Florent KRZAKALA\\
	et au sein de l'école doctorale physique en île de France\\[6pt]	
%
	Université Paris Diderot (Paris 7) Sorbonne Paris cité\\
	pour l'obtention du grade de Docteur ès Sciences\\
	spécialité physique théorique, par\\[6pt]
	\null \hspace{3em} Jean BARBIER\\[6pt]
%
\small
acceptée sur la proposition du jury:\\[6pt]
%
    Prof. Laurent DAUDET, examinateur\\
    Prof. Silvio FRANZ, examinateur\\
    Prof. Florent KRZAKALA, directeur\\
    Prof. Marc LELARGE, examinateur\\
    Prof. Nicolas MACRIS, rapporteur\\
    Prof. Marc M\'EZARD, examinateur\\ 
    Prof. Federico RICCI-TERSENGHI, examinateur\\
    Prof. David SAAD, rapporteur\\[6pt]               
%
Paris, \'Ecole Normale Supérieure, 2015.}
\end{tabular}
\end{center}
\vspace{2cm}
\end{titlepage}

==> images/ch_images/figures/tex/all_baboon_snr35.tex <==
TVAL3 Optimal & -15.92 & -17.27 & -19.65 & \textbf{-21.73} & \textbf{-23.72} & -25.77 \\ 
DC-AMP Optimal & \textbf{-16.18} & \textbf{-17.50} & \textbf{-19.75} & -21.61 & -23.70 & \textbf{-25.81} \\ 


==> images/ch_images/figures/tex/all_barbara_snr35.tex <==
TVAL3 Optimal & \textbf{-15.32} & \textbf{-16.30} & -17.80 & -19.67 & -22.01 & -24.52 \\ 
DC-AMP Optimal & -15.25 & -16.22 & \textbf{-17.94} & \textbf{-20.02} & \textbf{-22.46} & \textbf{-25.29} \\ 


==> images/ch_images/figures/tex/all_cameraman_snr35.tex <==
TVAL3 Optimal & -21.44 & -24.93 & -28.97 & -32.02 & -34.38 & -36.44 \\ 
DC-AMP Optimal & \textbf{-21.63} & \textbf{-25.02} & \textbf{-29.27} & \textbf{-32.70} & \textbf{-35.13} & \textbf{-36.90} \\ 


==> images/ch_images/figures/tex/all_lena_snr35.tex <==
TVAL3 Optimal & \textbf{-19.77} & -22.41 & \textbf{-25.63} & \textbf{-27.74} & -29.36 & -30.82 \\ 
DC-AMP Optimal & -19.32 & \textbf{-22.62} & -25.52 & -27.70 & \textbf{-29.42} & \textbf{-31.01} \\ 


==> images/ch_images/figures/tex/all_peppers_snr35.tex <==
TVAL3 Optimal & \textbf{-21.50} & \textbf{-24.17} & \textbf{-26.28} & \textbf{-27.52} & \textbf{-28.55} & -29.54 \\ 
DC-AMP Optimal & -21.24 & -23.72 & -26.18 & -27.46 & -28.51 & \textbf{-29.67} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr0.tex <==
TV-AL3 & \textbf{-2.57} & \textbf{-3.74} & -4.51 & -4.95 & -5.42 & -5.56 \\ 
ss-AMP (1D) & 1.91 & 2.17 & 2.84 & 2.60 & 2.52 & 2.48 \\ 
ss-AMP (1D) w/ Learning & -1.92 & -2.45 & -3.22 & -3.66 & -3.97 & -4.23 \\ 
TV-GaBP w/ Learning & -1.54 & -2.90 & \textbf{-4.94} & \textbf{-5.77} & \textbf{-6.40} & \textbf{-6.59} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr10.tex <==
TV-AL3 & -4.54 & -5.44 & -6.75 & -8.15 & \textbf{-9.08} & \textbf{-9.89} \\ 
ss-AMP (1D) & -1.53 & -2.52 & -3.85 & -3.11 & -3.85 & -4.43 \\ 
ss-AMP (1D) w/ Learning & -1.84 & -2.83 & -4.66 & -5.64 & -6.41 & -7.24 \\ 
TV-GaBP w/ Learning & \textbf{-6.44} & \textbf{-7.25} & \textbf{-8.03} & \textbf{-8.57} & -8.98 & -9.30 \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr15.tex <==
TV-AL3 & -4.98 & -6.12 & -7.99 & -9.60 & -10.96 & -12.13 \\ 
ss-AMP (1D) & -2.05 & -3.20 & -5.15 & -6.84 & -8.41 & -9.90 \\ 
ss-AMP (1D) w/ Learning & -2.11 & -3.23 & -5.16 & -6.84 & -8.41 & -9.89 \\ 
TV-GaBP w/ Learning & \textbf{-9.29} & \textbf{-10.49} & \textbf{-12.04} & \textbf{-12.96} & \textbf{-13.54} & \textbf{-13.98} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr20.tex <==
TV-AL3 & -5.30 & -6.60 & -8.74 & -10.56 & -12.25 & -13.81 \\ 
ss-AMP (1D) & -2.21 & -3.39 & -5.42 & -7.22 & -8.99 & -10.74 \\ 
ss-AMP (1D) w/ Learning & -2.26 & -3.42 & -5.43 & -7.21 & -8.98 & -10.72 \\ 
TV-GaBP w/ Learning & \textbf{-11.98} & \textbf{-13.53} & \textbf{-15.34} & \textbf{-16.54} & \textbf{-17.44} & \textbf{-18.12} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr25.tex <==
TV-AL3 & -5.34 & -6.66 & -8.86 & -10.83 & -12.67 & -14.48 \\ 
ss-AMP (1D) & -2.25 & -3.45 & -5.51 & -7.35 & -9.19 & -11.05 \\ 
ss-AMP (1D) w/ Learning & -2.31 & -3.48 & -5.52 & -7.33 & -9.17 & -11.03 \\ 
TV-GaBP w/ Learning & \textbf{-13.49} & \textbf{-15.20} & \textbf{-17.26} & \textbf{-18.75} & \textbf{-19.93} & \textbf{-21.03} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr30.tex <==
TV-AL3 & -5.35 & -6.67 & -8.90 & -10.91 & -12.82 & -14.74 \\ 
ss-AMP (1D) & -2.27 & -3.47 & -5.54 & -7.40 & -9.26 & -11.15 \\ 
ss-AMP (1D) w/ Learning & -2.33 & -3.50 & -5.54 & -7.38 & -9.24 & -11.12 \\ 
TV-GaBP w/ Learning & \textbf{-14.10} & \textbf{-15.89} & \textbf{-18.13} & \textbf{-19.79} & \textbf{-21.20} & \textbf{-22.62} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr35.tex <==
TV-AL3 & -5.37 & -6.70 & -8.94 & -10.98 & -12.90 & -14.87 \\ 
ss-AMP (1D) & -2.28 & -3.48 & -5.55 & -7.41 & -9.28 & -11.19 \\ 
ss-AMP (1D) w/ Learning & -2.33 & -3.51 & -5.55 & -7.39 & -9.26 & -11.16 \\ 
TV-GaBP w/ Learning & \textbf{-14.32} & \textbf{-16.17} & \textbf{-18.44} & \textbf{-20.19} & \textbf{-21.69} & \textbf{-23.25} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr40.tex <==
TV-AL3 & -5.40 & -6.73 & -8.95 & -10.99 & -12.94 & -14.93 \\ 
ss-AMP (1D) & -2.28 & -3.48 & -5.55 & -7.41 & -9.28 & -11.20 \\ 
ss-AMP (1D) w/ Learning & -2.33 & -3.51 & -5.55 & -7.39 & -9.26 & -11.17 \\ 
TV-GaBP w/ Learning & \textbf{-14.41} & \textbf{-16.24} & \textbf{-18.55} & \textbf{-20.32} & \textbf{-21.85} & \textbf{-23.48} \\ 


==> images/ch_images/figures/tex/old/all_baboon_snr5.tex <==
TV-AL3 & -3.94 & -4.68 & \textbf{-5.60} & \textbf{-6.12} & \textbf{-6.92} & \textbf{-7.30} \\ 
ss-AMP (1D) & -0.37 & -1.02 & -0.91 & -0.83 & -1.16 & -1.44 \\ 
ss-AMP (1D) w/ Learning & -1.23 & -3.02 & -4.24 & -4.78 & -5.27 & -5.70 \\ 
TV-GaBP w/ Learning & \textbf{-4.32} & \textbf{-6.14} & -5.58 & -5.09 & -4.60 & -4.55 \\ 


==> images/ch_images/figures/tex/old/all_baboon_snrInf.tex <==
TV-AL3 & -5.40 & -6.73 & -8.96 & -10.99 & -12.94 & -14.94 \\ 
ss-AMP (1D) & -2.28 & -3.48 & -5.55 & -7.41 & -9.29 & -11.20 \\ 
ss-AMP (1D) w/ Learning & -2.33 & -3.51 & -5.56 & -7.39 & -9.27 & -11.17 \\ 
TV-GaBP w/ Learning & \textbf{-14.44} & \textbf{-16.29} & \textbf{-18.60} & \textbf{-20.39} & \textbf{-21.93} & \textbf{-23.59} \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr0.tex <==
TV-AL3 & \textbf{-3.21} & \textbf{-4.74} & \textbf{-6.81} & \textbf{-7.60} & \textbf{-8.01} & \textbf{-8.04} \\ 
ss-AMP (1D) & 0.87 & 1.08 & 2.06 & 1.95 & 1.85 & 1.82 \\ 
ss-AMP (1D) w/ Learning & -2.32 & -3.10 & -4.26 & -5.05 & -5.62 & -6.10 \\ 
TV-GaBP w/ Learning & -1.61 & -2.95 & -4.74 & -5.33 & -5.29 & -2.40 \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr10.tex <==
TV-AL3 & \textbf{-6.81} & \textbf{-8.31} & \textbf{-8.94} & \textbf{-9.49} & \textbf{-9.79} & \textbf{-10.33} \\ 
ss-AMP (1D) & -3.66 & -4.99 & -6.20 & -5.20 & -5.72 & -6.04 \\ 
ss-AMP (1D) w/ Learning & -3.91 & -5.37 & -7.37 & -8.63 & -9.49 & -10.26 \\ 
TV-GaBP w/ Learning & -6.26 & -7.16 & -8.18 & -8.71 & -9.07 & -9.38 \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr15.tex <==
TV-AL3 & -8.05 & -8.83 & -9.73 & -10.80 & -11.91 & -13.05 \\ 
ss-AMP (1D) & -4.46 & -6.17 & -8.11 & -9.64 & -10.99 & -12.17 \\ 
ss-AMP (1D) w/ Learning & -4.52 & -6.21 & -8.12 & -9.64 & -11.01 & -12.19 \\ 
TV-GaBP w/ Learning & \textbf{-9.32} & \textbf{-10.57} & \textbf{-11.83} & \textbf{-12.63} & \textbf{-13.19} & \textbf{-13.65} \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr20.tex <==
TV-AL3 & -8.31 & -9.10 & -10.44 & -11.99 & -13.53 & -15.04 \\ 
ss-AMP (1D) & -4.71 & -6.53 & -8.69 & -10.45 & -12.14 & -13.71 \\ 
ss-AMP (1D) w/ Learning & -4.75 & -6.56 & -8.69 & -10.44 & -12.14 & -13.69 \\ 
TV-GaBP w/ Learning & \textbf{-11.72} & \textbf{-13.20} & \textbf{-14.56} & \textbf{-15.51} & \textbf{-16.25} & \textbf{-16.92} \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr25.tex <==
TV-AL3 & -8.40 & -9.21 & -10.70 & -12.44 & -14.39 & -16.44 \\ 
ss-AMP (1D) & -4.79 & -6.67 & -8.88 & -10.72 & -12.55 & -14.33 \\ 
ss-AMP (1D) w/ Learning & -4.83 & -6.69 & -8.88 & -10.71 & -12.54 & -14.30 \\ 
TV-GaBP w/ Learning & \textbf{-12.94} & \textbf{-14.52} & \textbf{-15.93} & \textbf{-16.97} & \textbf{-17.92} & \textbf{-18.80} \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr30.tex <==
TV-AL3 & -8.44 & -9.25 & -10.78 & -12.64 & -14.74 & -17.02 \\ 
ss-AMP (1D) & -4.83 & -6.70 & -8.94 & -10.83 & -12.69 & -14.55 \\ 
ss-AMP (1D) w/ Learning & -4.87 & -6.72 & -8.94 & -10.81 & -12.69 & -14.51 \\ 
TV-GaBP w/ Learning & \textbf{-13.40} & \textbf{-15.04} & \textbf{-16.48} & \textbf{-17.58} & \textbf{-18.62} & \textbf{-19.61} \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr35.tex <==
TV-AL3 & -8.44 & -9.28 & -10.83 & -12.70 & -14.85 & -17.25 \\ 
ss-AMP (1D) & -4.83 & -6.71 & -8.97 & -10.85 & -12.74 & -14.62 \\ 
ss-AMP (1D) w/ Learning & -4.87 & -6.73 & -8.96 & -10.84 & -12.73 & -14.58 \\ 
TV-GaBP w/ Learning & \textbf{-13.57} & \textbf{-15.23} & \textbf{-16.66} & \textbf{-17.80} & \textbf{-18.87} & \textbf{-19.92} \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr40.tex <==
TV-AL3 & -8.44 & -9.32 & -10.86 & -12.73 & -14.92 & -17.35 \\ 
ss-AMP (1D) & -4.83 & -6.72 & -8.97 & -10.86 & -12.76 & -14.64 \\ 
ss-AMP (1D) w/ Learning & -4.87 & -6.74 & -8.97 & -10.85 & -12.75 & -14.60 \\ 
TV-GaBP w/ Learning & \textbf{-13.62} & \textbf{-15.28} & \textbf{-16.72} & \textbf{-17.87} & \textbf{-18.95} & \textbf{-20.01} \\ 


==> images/ch_images/figures/tex/old/all_barbara_snr5.tex <==
TV-AL3 & \textbf{-5.51} & \textbf{-6.91} & \textbf{-8.15} & \textbf{-8.57} & \textbf{-8.81} & \textbf{-9.08} \\ 
ss-AMP (1D) & -1.94 & -2.78 & -2.87 & -2.04 & -2.24 & -2.40 \\ 
ss-AMP (1D) w/ Learning & -2.97 & -5.07 & -6.56 & -7.41 & -8.04 & -8.53 \\ 
TV-GaBP w/ Learning & -4.09 & -5.44 & -4.72 & -4.54 & -4.57 & -4.75 \\ 


==> images/ch_images/figures/tex/old/all_barbara_snrInf.tex <==
TV-AL3 & -8.43 & -9.30 & -10.87 & -12.74 & -14.94 & -17.35 \\ 
ss-AMP (1D) & -4.83 & -6.72 & -8.98 & -10.87 & -12.76 & -14.65 \\ 
ss-AMP (1D) w/ Learning & -4.87 & -6.74 & -8.97 & -10.85 & -12.75 & -14.61 \\ 
TV-GaBP w/ Learning & \textbf{-13.66} & \textbf{-15.31} & \textbf{-16.75} & \textbf{-17.90} & \textbf{-18.99} & \textbf{-20.06} \\ 


==> images/ch_images/figures/tex/old/all_boats_snr0.tex <==
TV-AL3 & \textbf{-3.39} & \textbf{-5.01} & \textbf{-6.81} & \textbf{-7.49} & \textbf{-8.22} & \textbf{-8.71} \\ 
ss-AMP (1D) & 1.35 & 1.46 & 2.24 & 2.13 & 2.07 & 2.12 \\ 
ss-AMP (1D) w/ Learning & -1.89 & -2.50 & -3.50 & -4.29 & -5.01 & -5.70 \\ 
TV-GaBP w/ Learning & -1.52 & -2.88 & -4.62 & -5.62 & -5.98 & -5.76 \\ 


==> images/ch_images/figures/tex/old/all_boats_snr10.tex <==
TV-AL3 & \textbf{-6.71} & \textbf{-8.55} & \textbf{-10.77} & \textbf{-11.67} & \textbf{-12.16} & \textbf{-12.76} \\ 
ss-AMP (1D) & -2.91 & -4.99 & -6.78 & -5.61 & -5.96 & -6.15 \\ 
ss-AMP (1D) w/ Learning & -3.04 & -5.18 & -7.10 & -9.29 & -10.33 & -11.23 \\ 
TV-GaBP w/ Learning & -6.37 & -7.23 & -8.18 & -8.77 & -9.23 & -9.45 \\ 


==> images/ch_images/figures/tex/old/all_boats_snr15.tex <==
TV-AL3 & -7.85 & -10.34 & -12.40 & \textbf{-13.69} & \textbf{-14.33} & \textbf{-15.20} \\ 
ss-AMP (1D) & -3.62 & -6.11 & -9.07 & -10.89 & -12.29 & -13.30 \\ 
ss-AMP (1D) w/ Learning & -3.64 & -6.12 & -9.08 & -10.91 & -12.32 & -13.33 \\ 
TV-GaBP w/ Learning & \textbf{-9.55} & \textbf{-10.93} & \textbf{-12.46} & -13.25 & -13.77 & -14.17 \\ 


==> images/ch_images/figures/tex/old/all_boats_snr20.tex <==
TV-AL3 & -9.29 & -11.24 & -13.53 & -15.02 & -16.08 & -16.91 \\ 
ss-AMP (1D) & -3.85 & -6.49 & -9.77 & -12.03 & -13.87 & -15.40 \\ 
ss-AMP (1D) w/ Learning & -3.86 & -6.48 & -9.76 & -12.03 & -13.86 & -15.39 \\ 
TV-GaBP w/ Learning & \textbf{-12.52} & \textbf{-14.30} & \textbf{-16.10} & \textbf{-17.15} & \textbf{-17.91} & \textbf{-18.43} \\ 


==> images/ch_images/figures/tex/old/all_boats_snr25.tex <==
TV-AL3 & -9.44 & -11.53 & -14.17 & -15.93 & -17.30 & -18.51 \\ 
ss-AMP (1D) & -3.90 & -6.61 & -10.03 & -12.45 & -14.50 & -16.36 \\ 
ss-AMP (1D) w/ Learning & -3.91 & -6.60 & -10.02 & -12.43 & -14.50 & -16.33 \\ 
TV-GaBP w/ Learning & \textbf{-14.17} & \textbf{-16.28} & \textbf{-18.39} & \textbf{-19.78} & \textbf{-20.88} & \textbf{-21.64} \\ 


==> images/ch_images/figures/tex/old/all_boats_snr30.tex <==
TV-AL3 & -9.46 & -11.62 & -14.40 & -16.26 & -17.87 & -19.24 \\ 
ss-AMP (1D) & -3.93 & -6.65 & -10.11 & -12.59 & -14.73 & -16.72 \\ 
ss-AMP (1D) w/ Learning & -3.93 & -6.64 & -10.10 & -12.57 & -14.72 & -16.69 \\ 
TV-GaBP w/ Learning & \textbf{-14.90} & \textbf{-17.26} & \textbf{-19.59} & \textbf{-21.13} & \textbf{-22.54} & \textbf{-23.47} \\ 


==> images/ch_images/figures/tex/old/all_boats_snr35.tex <==
TV-AL3 & -9.45 & -11.65 & -14.46 & -16.38 & -18.04 & -19.46 \\ 
ss-AMP (1D) & -3.93 & -6.66 & -10.14 & -12.63 & -14.81 & -16.84 \\ 
ss-AMP (1D) w/ Learning & -3.94 & -6.65 & -10.13 & -12.62 & -14.80 & -16.81 \\ 
TV-GaBP w/ Learning & \textbf{-15.17} & \textbf{-17.57} & \textbf{-20.02} & \textbf{-21.68} & \textbf{-23.23} & \textbf{-24.25} \\ 


==> images/ch_images/figures/tex/old/all_boats_snr40.tex <==
TV-AL3 & -9.39 & -11.66 & -14.50 & -16.45 & -18.14 & -19.60 \\ 
ss-AMP (1D) & -3.93 & -6.66 & -10.14 & -12.65 & -14.83 & -16.88 \\ 
ss-AMP (1D) w/ Learning & -3.94 & -6.65 & -10.13 & -12.63 & -14.82 & -16.84 \\ 
TV-GaBP w/ Learning & \textbf{-15.26} & \textbf{-17.66} & \textbf{-20.17} & \textbf{-21.86} & \textbf{-23.48} & \textbf{-24.55} \\ 


==> images/ch_images/figures/tex/old/all_boats_snr5.tex <==
TV-AL3 & \textbf{-5.41} & \textbf{-6.84} & \textbf{-8.53} & \textbf{-9.61} & \textbf{-10.00} & \textbf{-10.19} \\ 
ss-AMP (1D) & -1.40 & -2.69 & -2.10 & -2.04 & -2.21 & -2.20 \\ 
ss-AMP (1D) w/ Learning & -2.07 & -4.37 & -6.26 & -7.44 & -8.36 & -9.13 \\ 
TV-GaBP w/ Learning & -4.27 & -5.94 & -5.05 & -4.66 & -4.49 & -4.58 \\ 


==> images/ch_images/figures/tex/old/all_boats_snrInf.tex <==
TV-AL3 & -9.40 & -11.66 & -14.50 & -16.47 & -18.17 & -19.63 \\ 
ss-AMP (1D) & -3.93 & -6.66 & -10.15 & -12.65 & -14.84 & -16.90 \\ 
ss-AMP (1D) w/ Learning & -3.94 & -6.66 & -10.14 & -12.64 & -14.83 & -16.86 \\ 
TV-GaBP w/ Learning & \textbf{-15.31} & \textbf{-17.71} & \textbf{-20.24} & \textbf{-21.94} & \textbf{-23.59} & \textbf{-24.69} \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr0.tex <==
TV-AL3 & \textbf{-4.92} & \textbf{-7.13} & \textbf{-9.26} & \textbf{-10.57} & \textbf{-11.10} & \textbf{-11.50} \\ 
ss-AMP (1D) & 0.39 & 0.68 & 1.66 & 1.63 & 1.59 & 1.61 \\ 
ss-AMP (1D) w/ Learning & -3.62 & -4.61 & -5.95 & -6.91 & -7.79 & -8.39 \\ 
TV-GaBP w/ Learning & -1.77 & -3.11 & -4.93 & -5.66 & -5.74 & -5.25 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr10.tex <==
TV-AL3 & \textbf{-10.00} & \textbf{-11.76} & \textbf{-14.34} & \textbf{-15.44} & \textbf{-15.48} & \textbf{-15.27} \\ 
ss-AMP (1D) & -5.40 & -7.10 & -8.43 & -6.99 & -7.04 & -7.11 \\ 
ss-AMP (1D) w/ Learning & -5.65 & -7.40 & -10.74 & -12.54 & -13.43 & -14.22 \\ 
TV-GaBP w/ Learning & -6.51 & -7.47 & -8.53 & -9.11 & -9.47 & -9.72 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr15.tex <==
TV-AL3 & \textbf{-11.91} & \textbf{-14.46} & \textbf{-17.06} & \textbf{-17.86} & \textbf{-18.26} & \textbf{-18.14} \\ 
ss-AMP (1D) & -6.55 & -9.04 & -11.73 & -13.25 & -14.27 & -14.89 \\ 
ss-AMP (1D) w/ Learning & -6.61 & -9.07 & -11.77 & -13.29 & -14.34 & -15.01 \\ 
TV-GaBP w/ Learning & -9.78 & -11.31 & -12.88 & -13.72 & -14.21 & -14.55 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr20.tex <==
TV-AL3 & \textbf{-14.59} & \textbf{-16.77} & \textbf{-18.65} & \textbf{-19.44} & \textbf{-19.87} & \textbf{-20.12} \\ 
ss-AMP (1D) & -7.01 & -9.82 & -13.19 & -15.50 & -17.24 & -18.61 \\ 
ss-AMP (1D) w/ Learning & -7.05 & -9.84 & -13.21 & -15.49 & -17.25 & -18.61 \\ 
TV-GaBP w/ Learning & -12.62 & -14.66 & -16.71 & -17.87 & -18.63 & -19.12 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr25.tex <==
TV-AL3 & \textbf{-15.06} & \textbf{-17.94} & \textbf{-20.88} & \textbf{-22.59} & \textbf{-23.53} & \textbf{-24.22} \\ 
ss-AMP (1D) & -7.14 & -10.10 & -13.78 & -16.49 & -18.82 & -21.04 \\ 
ss-AMP (1D) w/ Learning & -7.18 & -10.10 & -13.79 & -16.47 & -18.79 & -20.88 \\ 
TV-GaBP w/ Learning & -14.15 & -16.67 & -19.24 & -20.85 & -22.10 & -22.85 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr30.tex <==
TV-AL3 & \textbf{-15.30} & \textbf{-18.34} & \textbf{-22.05} & \textbf{-24.49} & \textbf{-26.30} & \textbf{-27.73} \\ 
ss-AMP (1D) & -7.19 & -10.19 & -13.98 & -16.86 & -19.48 & -22.23 \\ 
ss-AMP (1D) w/ Learning & -7.23 & -10.20 & -13.99 & -16.84 & -19.43 & -21.92 \\ 
TV-GaBP w/ Learning & -14.75 & -17.55 & -20.52 & -22.51 & -24.24 & -25.33 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr35.tex <==
TV-AL3 & \textbf{-15.38} & \textbf{-18.57} & \textbf{-22.53} & \textbf{-25.52} & \textbf{-27.78} & \textbf{-29.74} \\ 
ss-AMP (1D) & -7.21 & -10.22 & -14.05 & -16.99 & -19.70 & -22.68 \\ 
ss-AMP (1D) w/ Learning & -7.25 & -10.23 & -14.05 & -16.97 & -19.63 & -22.31 \\ 
TV-GaBP w/ Learning & -14.98 & -17.93 & -21.04 & -23.21 & -25.24 & -26.54 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr40.tex <==
TV-AL3 & \textbf{-15.16} & \textbf{-18.61} & \textbf{-22.76} & \textbf{-25.92} & \textbf{-28.50} & \textbf{-30.83} \\ 
ss-AMP (1D) & -7.21 & -10.23 & -14.07 & -17.03 & -19.78 & -22.83 \\ 
ss-AMP (1D) w/ Learning & -7.25 & -10.24 & -14.07 & -17.01 & -19.71 & -22.44 \\ 
TV-GaBP w/ Learning & -15.04 & -18.02 & -21.21 & -23.45 & -25.60 & -27.00 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snr5.tex <==
TV-AL3 & \textbf{-6.49} & \textbf{-9.75} & \textbf{-11.33} & \textbf{-12.57} & \textbf{-13.43} & \textbf{-12.87} \\ 
ss-AMP (1D) & -3.00 & -3.88 & -3.70 & -2.85 & -2.90 & -2.87 \\ 
ss-AMP (1D) w/ Learning & -4.16 & -6.58 & -8.99 & -10.16 & -11.02 & -11.68 \\ 
TV-GaBP w/ Learning & -4.34 & -5.84 & -5.03 & -4.76 & -4.74 & -4.89 \\ 


==> images/ch_images/figures/tex/old/all_cameraman_snrInf.tex <==
TV-AL3 & \textbf{-15.23} & \textbf{-18.57} & \textbf{-22.82} & \textbf{-26.12} & \textbf{-28.89} & \textbf{-31.51} \\ 
ss-AMP (1D) & -7.21 & -10.24 & -14.08 & -17.05 & -19.82 & -22.91 \\ 
ss-AMP (1D) w/ Learning & -7.25 & -10.24 & -14.08 & -17.03 & -19.75 & -22.50 \\ 
TV-GaBP w/ Learning & -15.08 & -18.08 & -21.29 & -23.57 & -25.79 & -27.23 \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr0.tex <==
TV-AL3 & \textbf{-4.51} & \textbf{-6.63} & \textbf{-8.01} & \textbf{-8.85} & \textbf{-9.60} & \textbf{-9.67} \\ 
ss-AMP (1D) & 0.42 & 0.84 & 1.90 & 1.82 & 1.79 & 1.82 \\ 
ss-AMP (1D) w/ Learning & -3.27 & -4.28 & -5.81 & -6.68 & -7.34 & -7.77 \\ 
TV-GaBP w/ Learning & -1.65 & -2.89 & -4.69 & -5.23 & -2.85 & -1.99 \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr10.tex <==
TV-AL3 & \textbf{-8.64} & \textbf{-10.14} & \textbf{-11.75} & \textbf{-12.30} & \textbf{-12.81} & \textbf{-12.97} \\ 
ss-AMP (1D) & -5.21 & -6.43 & -7.42 & -6.01 & -6.27 & -6.44 \\ 
ss-AMP (1D) w/ Learning & -5.45 & -6.74 & -8.63 & -10.37 & -11.25 & -11.99 \\ 
TV-GaBP w/ Learning & -6.33 & -7.31 & -8.42 & -8.95 & -9.31 & -9.61 \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr15.tex <==
TV-AL3 & \textbf{-9.93} & \textbf{-11.59} & \textbf{-13.45} & \textbf{-14.29} & \textbf{-14.88} & \textbf{-15.28} \\ 
ss-AMP (1D) & -6.31 & -8.17 & -10.25 & -11.53 & -12.55 & -13.29 \\ 
ss-AMP (1D) w/ Learning & -6.36 & -8.19 & -10.28 & -11.56 & -12.58 & -13.32 \\ 
TV-GaBP w/ Learning & -9.63 & -11.02 & -12.58 & -13.41 & -13.91 & -14.29 \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr20.tex <==
TV-AL3 & -11.09 & -12.62 & -14.43 & -15.63 & -16.58 & -17.38 \\ 
ss-AMP (1D) & -6.74 & -8.83 & -11.23 & -12.87 & -14.24 & -15.45 \\ 
ss-AMP (1D) w/ Learning & -6.78 & -8.85 & -11.24 & -12.88 & -14.24 & -15.45 \\ 
TV-GaBP w/ Learning & \textbf{-12.34} & \textbf{-14.17} & \textbf{-16.03} & \textbf{-17.14} & \textbf{-17.85} & \textbf{-18.43} \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr25.tex <==
TV-AL3 & -11.28 & -12.96 & -15.09 & -16.63 & -17.91 & -19.12 \\ 
ss-AMP (1D) & -6.86 & -9.01 & -11.58 & -13.38 & -14.93 & -16.40 \\ 
ss-AMP (1D) w/ Learning & -6.89 & -9.02 & -11.59 & -13.38 & -14.92 & -16.39 \\ 
TV-GaBP w/ Learning & \textbf{-13.73} & \textbf{-15.92} & \textbf{-18.07} & \textbf{-19.14} & \textbf{-20.56} & \textbf{-21.40} \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr30.tex <==
TV-AL3 & -11.33 & -13.09 & -15.32 & -17.04 & -18.46 & -19.91 \\ 
ss-AMP (1D) & -6.89 & -9.09 & -11.70 & -13.55 & -15.20 & -16.77 \\ 
ss-AMP (1D) w/ Learning & -6.92 & -9.10 & -11.70 & -13.55 & -15.18 & -16.75 \\ 
TV-GaBP w/ Learning & \textbf{-14.30} & \textbf{-16.64} & \textbf{-19.02} & \textbf{-20.12} & \textbf{-21.95} & \textbf{-23.03} \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr35.tex <==
TV-AL3 & -11.34 & -13.12 & -15.46 & -17.12 & -18.70 & -20.22 \\ 
ss-AMP (1D) & -6.91 & -9.10 & -11.74 & -13.61 & -15.28 & -16.89 \\ 
ss-AMP (1D) w/ Learning & -6.94 & -9.11 & -11.75 & -13.61 & -15.26 & -16.88 \\ 
TV-GaBP w/ Learning & \textbf{-14.52} & \textbf{-16.93} & \textbf{-19.37} & \textbf{-20.49} & \textbf{-22.52} & \textbf{-23.72} \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr40.tex <==
TV-AL3 & -11.31 & -13.14 & -15.49 & -17.24 & -18.77 & -20.36 \\ 
ss-AMP (1D) & -6.92 & -9.11 & -11.75 & -13.63 & -15.30 & -16.93 \\ 
ss-AMP (1D) w/ Learning & -6.94 & -9.12 & -11.76 & -13.63 & -15.29 & -16.92 \\ 
TV-GaBP w/ Learning & \textbf{-14.57} & \textbf{-17.01} & \textbf{-19.49} & \textbf{-20.61} & \textbf{-22.71} & \textbf{-23.96} \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snr5.tex <==
TV-AL3 & \textbf{-6.93} & \textbf{-8.47} & \textbf{-9.95} & \textbf{-10.70} & \textbf{-10.79} & \textbf{-10.76} \\ 
ss-AMP (1D) & -2.89 & -3.58 & -3.17 & -2.41 & -2.50 & -2.49 \\ 
ss-AMP (1D) w/ Learning & -3.91 & -6.24 & -8.10 & -8.94 & -9.60 & -10.18 \\ 
TV-GaBP w/ Learning & -4.15 & -5.30 & -4.68 & -4.55 & -4.63 & -4.82 \\ 


==> images/ch_images/figures/tex/old/all_goldhill_snrInf.tex <==
TV-AL3 & -11.31 & -13.15 & -15.49 & -17.26 & -18.80 & -20.41 \\ 
ss-AMP (1D) & -6.92 & -9.11 & -11.76 & -13.64 & -15.32 & -16.95 \\ 
ss-AMP (1D) w/ Learning & -6.95 & -9.12 & -11.76 & -13.64 & -15.30 & -16.93 \\ 
TV-GaBP w/ Learning & \textbf{-14.62} & \textbf{-17.06} & \textbf{-19.54} & \textbf{-20.67} & \textbf{-22.81} & \textbf{-24.08} \\ 


==> images/ch_images/figures/tex/old/all_lena_snr0.tex <==
TV-AL3 & \textbf{-3.32} & \textbf{-6.00} & \textbf{-8.43} & \textbf{-9.37} & \textbf{-10.11} & \textbf{-10.42} \\ 
ss-AMP (1D) & 0.51 & 0.78 & 1.87 & 1.79 & 1.76 & 1.80 \\ 
ss-AMP (1D) w/ Learning & -2.91 & -3.85 & -5.35 & -6.41 & -7.26 & -8.00 \\ 
TV-GaBP w/ Learning & -1.64 & -2.94 & -4.76 & -5.39 & -5.28 & -2.25 \\ 


==> images/ch_images/figures/tex/old/all_lena_snr10.tex <==
TV-AL3 & \textbf{-8.38} & \textbf{-10.95} & \textbf{-12.81} & \textbf{-13.78} & \textbf{-13.73} & \textbf{-14.12} \\ 
ss-AMP (1D) & -5.04 & -6.80 & -8.04 & -6.61 & -6.75 & -6.85 \\ 
ss-AMP (1D) w/ Learning & -5.22 & -7.10 & -9.85 & -11.71 & -12.64 & -13.42 \\ 
TV-GaBP w/ Learning & -6.40 & -7.38 & -8.46 & -8.97 & -9.33 & -9.62 \\ 


==> images/ch_images/figures/tex/old/all_lena_snr15.tex <==
TV-AL3 & \textbf{-10.69} & \textbf{-12.71} & \textbf{-14.79} & \textbf{-15.90} & \textbf{-16.40} & \textbf{-16.82} \\ 
ss-AMP (1D) & -6.08 & -8.54 & -11.13 & -12.65 & -13.68 & -14.33 \\ 
ss-AMP (1D) w/ Learning & -6.10 & -8.57 & -11.15 & -12.69 & -13.72 & -14.39 \\ 
TV-GaBP w/ Learning & -9.72 & -11.22 & -12.72 & -13.58 & -14.05 & -14.41 \\ 


==> images/ch_images/figures/tex/old/all_lena_snr20.tex <==
TV-AL3 & -12.15 & -14.20 & -16.31 & -17.42 & -18.15 & -18.65 \\ 
ss-AMP (1D) & -6.46 & -9.23 & -12.38 & -14.47 & -16.04 & -17.29 \\ 
ss-AMP (1D) w/ Learning & -6.48 & -9.23 & -12.38 & -14.47 & -16.05 & -17.31 \\ 
TV-GaBP w/ Learning & \textbf{-12.67} & \textbf{-14.60} & \textbf{-16.53} & \textbf{-17.64} & \textbf{-18.35} & \textbf{-18.83} \\ 


==> images/ch_images/figures/tex/old/all_lena_snr25.tex <==
TV-AL3 & -12.40 & -14.79 & -17.45 & -19.02 & -20.23 & -21.16 \\ 
ss-AMP (1D) & -6.59 & -9.47 & -12.84 & -15.23 & -17.18 & -18.88 \\ 
ss-AMP (1D) w/ Learning & -6.60 & -9.48 & -12.83 & -15.22 & -17.17 & -18.86 \\ 
TV-GaBP w/ Learning & \textbf{-14.28} & \textbf{-16.63} & \textbf{-18.99} & \textbf{-20.50} & \textbf{-21.56} & \textbf{-22.29} \\ 


==> images/ch_images/figures/tex/old/all_lena_snr30.tex <==
TV-AL3 & -12.48 & -14.98 & -17.88 & -19.77 & -21.26 & -22.53 \\ 
ss-AMP (1D) & -6.63 & -9.55 & -13.00 & -15.51 & -17.61 & -19.55 \\ 
ss-AMP (1D) w/ Learning & -6.64 & -9.55 & -12.99 & -15.49 & -17.59 & -19.51 \\ 
TV-GaBP w/ Learning & \textbf{-14.94} & \textbf{-17.58} & \textbf{-20.17} & \textbf{-22.04} & \textbf{-23.45} & \textbf{-24.44} \\ 


==> images/ch_images/figures/tex/old/all_lena_snr35.tex <==
TV-AL3 & -12.47 & -15.01 & -18.02 & -20.03 & -21.68 & -23.07 \\ 
ss-AMP (1D) & -6.64 & -9.57 & -13.05 & -15.60 & -17.75 & -19.78 \\ 
ss-AMP (1D) w/ Learning & -6.65 & -9.57 & -13.04 & -15.58 & -17.73 & -19.74 \\ 
TV-GaBP w/ Learning & \textbf{-15.14} & \textbf{-17.94} & \textbf{-20.65} & \textbf{-22.69} & \textbf{-24.30} & \textbf{-25.43} \\ 


==> images/ch_images/figures/tex/old/all_lena_snr40.tex <==
TV-AL3 & -12.45 & -15.07 & -18.09 & -20.11 & -21.85 & -23.32 \\ 
ss-AMP (1D) & -6.65 & -9.58 & -13.07 & -15.62 & -17.80 & -19.85 \\ 
ss-AMP (1D) w/ Learning & -6.66 & -9.58 & -13.06 & -15.60 & -17.78 & -19.81 \\ 
TV-GaBP w/ Learning & \textbf{-15.24} & \textbf{-18.04} & \textbf{-20.81} & \textbf{-22.90} & \textbf{-24.59} & \textbf{-25.79} \\ 


==> images/ch_images/figures/tex/old/all_lena_snr5.tex <==
TV-AL3 & \textbf{-6.69} & \textbf{-8.97} & \textbf{-10.57} & \textbf{-11.29} & \textbf{-11.78} & \textbf{-11.59} \\ 
ss-AMP (1D) & -2.79 & -3.70 & -3.24 & -2.59 & -2.65 & -2.63 \\ 
ss-AMP (1D) w/ Learning & -3.69 & -6.18 & -8.54 & -9.72 & -10.49 & -11.08 \\ 
TV-GaBP w/ Learning & -4.17 & -5.51 & -4.74 & -4.57 & -4.61 & -4.79 \\ 


==> images/ch_images/figures/tex/old/all_lena_snrInf.tex <==
TV-AL3 & -12.40 & -15.06 & -18.10 & -20.16 & -21.92 & -23.45 \\ 
ss-AMP (1D) & -6.65 & -9.58 & -13.08 & -15.64 & -17.83 & -19.89 \\ 
ss-AMP (1D) w/ Learning & -6.66 & -9.59 & -13.06 & -15.62 & -17.80 & -19.84 \\ 
TV-GaBP w/ Learning & \textbf{-15.29} & \textbf{-18.10} & \textbf{-20.89} & \textbf{-23.01} & \textbf{-24.73} & \textbf{-25.97} \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr0.tex <==
TV-AL3 & \textbf{-3.44} & \textbf{-6.28} & \textbf{-8.99} & \textbf{-10.04} & \textbf{-10.01} & \textbf{-10.90} \\ 
ss-AMP (1D) & 0.54 & 0.70 & 1.74 & 1.68 & 1.64 & 1.66 \\ 
ss-AMP (1D) w/ Learning & -2.33 & -3.19 & -4.45 & -5.53 & -6.44 & -7.19 \\ 
TV-GaBP w/ Learning & -1.74 & -3.16 & -5.07 & -6.02 & -6.48 & -6.48 \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr10.tex <==
TV-AL3 & \textbf{-9.09} & \textbf{-11.84} & \textbf{-13.35} & \textbf{-14.62} & \textbf{-14.44} & \textbf{-14.73} \\ 
ss-AMP (1D) & -4.72 & -6.76 & -8.14 & -6.64 & -6.81 & -6.87 \\ 
ss-AMP (1D) w/ Learning & -4.85 & -7.05 & -9.07 & -11.59 & -12.69 & -13.43 \\ 
TV-GaBP w/ Learning & -6.67 & -7.61 & -8.49 & -9.03 & -9.32 & -9.63 \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr15.tex <==
TV-AL3 & \textbf{-10.88} & \textbf{-14.04} & \textbf{-15.49} & \textbf{-16.38} & \textbf{-16.75} & \textbf{-16.88} \\ 
ss-AMP (1D) & -5.69 & -8.48 & -11.09 & -12.43 & -13.40 & -14.11 \\ 
ss-AMP (1D) w/ Learning & -5.71 & -8.49 & -11.14 & -12.49 & -13.50 & -14.26 \\ 
TV-GaBP w/ Learning & -9.86 & -11.24 & -12.76 & -13.58 & -14.11 & -14.40 \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr20.tex <==
TV-AL3 & \textbf{-13.62} & \textbf{-15.44} & -16.65 & -17.32 & -17.79 & -18.17 \\ 
ss-AMP (1D) & -6.06 & -9.15 & -12.32 & -14.20 & -15.68 & -17.08 \\ 
ss-AMP (1D) w/ Learning & -6.06 & -9.13 & -12.34 & -14.21 & -15.71 & -17.07 \\ 
TV-GaBP w/ Learning & -12.82 & -14.85 & \textbf{-16.68} & \textbf{-17.72} & \textbf{-18.37} & \textbf{-18.80} \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr25.tex <==
TV-AL3 & -13.88 & -16.05 & -17.78 & -18.72 & -19.46 & -20.20 \\ 
ss-AMP (1D) & -6.17 & -9.40 & -12.78 & -14.92 & -16.74 & -18.78 \\ 
ss-AMP (1D) w/ Learning & -6.17 & -9.38 & -12.79 & -14.92 & -16.72 & -18.55 \\ 
TV-GaBP w/ Learning & \textbf{-14.53} & \textbf{-16.96} & \textbf{-19.25} & \textbf{-20.66} & \textbf{-21.59} & \textbf{-22.25} \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr30.tex <==
TV-AL3 & -13.94 & -16.26 & -18.15 & -19.21 & -20.20 & -21.20 \\ 
ss-AMP (1D) & -6.21 & -9.48 & -12.94 & -15.18 & -17.13 & -19.50 \\ 
ss-AMP (1D) w/ Learning & -6.20 & -9.45 & -12.94 & -15.18 & -17.10 & -19.14 \\ 
TV-GaBP w/ Learning & \textbf{-15.21} & \textbf{-17.92} & \textbf{-20.56} & \textbf{-22.27} & \textbf{-23.49} & \textbf{-24.37} \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr35.tex <==
TV-AL3 & -14.00 & -16.37 & -18.26 & -19.45 & -20.45 & -21.57 \\ 
ss-AMP (1D) & -6.22 & -9.50 & -13.00 & -15.27 & -17.27 & -19.75 \\ 
ss-AMP (1D) w/ Learning & -6.22 & -9.48 & -13.00 & -15.26 & -17.24 & -19.34 \\ 
TV-GaBP w/ Learning & \textbf{-15.48} & \textbf{-18.29} & \textbf{-21.04} & \textbf{-22.95} & \textbf{-24.34} & \textbf{-25.34} \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr40.tex <==
TV-AL3 & -14.00 & -16.40 & -18.35 & -19.57 & -20.57 & -21.73 \\ 
ss-AMP (1D) & -6.23 & -9.51 & -13.01 & -15.30 & -17.32 & -19.85 \\ 
ss-AMP (1D) w/ Learning & -6.22 & -9.49 & -13.02 & -15.30 & -17.28 & -19.41 \\ 
TV-GaBP w/ Learning & \textbf{-15.55} & \textbf{-18.41} & \textbf{-21.22} & \textbf{-23.17} & \textbf{-24.62} & \textbf{-25.70} \\ 


==> images/ch_images/figures/tex/old/all_peppers_snr5.tex <==
TV-AL3 & \textbf{-6.98} & \textbf{-9.01} & \textbf{-11.60} & \textbf{-12.32} & \textbf{-12.50} & \textbf{-12.54} \\ 
ss-AMP (1D) & -2.74 & -3.77 & -3.62 & -2.70 & -2.76 & -2.74 \\ 
ss-AMP (1D) w/ Learning & -3.64 & -6.02 & -8.22 & -9.47 & -10.42 & -11.07 \\ 
TV-GaBP w/ Learning & -4.48 & -6.40 & -5.55 & -5.09 & -4.74 & -4.75 \\ 


==> images/ch_images/figures/tex/old/all_peppers_snrInf.tex <==
TV-AL3 & -14.03 & -16.41 & -18.37 & -19.59 & -20.61 & -21.79 \\ 
ss-AMP (1D) & -6.23 & -9.51 & -13.02 & -15.31 & -17.34 & -19.89 \\ 
ss-AMP (1D) w/ Learning & -6.22 & -9.49 & -13.03 & -15.31 & -17.30 & -19.44 \\ 
TV-GaBP w/ Learning & \textbf{-15.59} & \textbf{-18.48} & \textbf{-21.30} & \textbf{-23.29} & \textbf{-24.77} & \textbf{-25.87} \\ 


==> main/listOfSymbols.tex <==
\markboth{List of symbols and acronyms}{List of symbols and acronyms}
\addcontentsline{toc}{chapter}{List of symbols and acronyms}

\chapter*{List of symbols and acronyms}

\begin{flalign*}
a \ \ \ \ &: \ \ \ \ \txt{a generic quantity, usually a scalar if not precised further.}&\\
\tbf a \ \ \ \ &:\ \ \ \ \txt{a vector.} \\
\tbf A\ \ \ \ &:\ \ \ \ \txt{a matrix.} \\
a_{i} = (\tbf a)_i \ \ \ \ &:\ \ \ \ \txt{the $i^{th}$ component of $\tbf{a}$. The two notations are equivalent.}\\
A_{ij}\ \ \ \ &:\ \ \ \ \txt{the element at the $i^{th}$ line and $j^{th}$ column of}\ \tbf{A}. \\
\tbf A_{i,\bullet}\ \ \ \ &:\ \ \ \ \txt{the $i^{th}$ line of $\tbf A$.} \\
\tbf A_{\bullet,i}\ \ \ \ &:\ \ \ \ \txt{the $i^{th}$ column of $\tbf A$.} \\
\bs \ \ \ \ &:\ \ \ \ \txt{generally the signal or message to infer.} \\
\bx \ \ \ \ &:\ \ \ \ \txt{an intermediate variable for estimating $\bs$.} \\
\hat \bx\ \ \ \ &:\ \ \ \ \txt{the final estimate of the signal $\bs$.} \\
\by\ \ \ \ &:\ \ \ \ \txt{the measurement vector or codeword.} \\
\bF\ \ \ \ &:\ \ \ \ \txt{the measurement or coding operator.} \\
\hat a\ \ \ \ &:\ \ \ \ \txt{the estimate of the quantity $a$.} \\
K\ \ \ \ &:\ \ \ \ \txt{number of non zero components in the sparse signal} \ \bs.\\
N\ \ \ \ &:\ \ \ \ \txt{number of scalar components of the signal or message to reconstruct} \ \bs.\\
L\ \ \ \ &:\ \ \ \ \txt{number of vector components of the signal or message to reconstruct} \ \bs.\\
M\ \ \ \ &:\ \ \ \ \txt{number of scalar components of the measure or codeword} \ \by. \\
\defeq\ \ \ \ &:\ \ \ \ \txt{equal by definition.} \\
\rho \defeq K/N \ \ \ \ &:\ \ \ \ \txt{density of non zero components of} \ \bs. \\
\alpha \defeq M/N \ \ \ \ &:\ \ \ \ \txt{the measurement rate.}
\end{flalign*}
%
%
%
%
%
%
\begin{flalign*}
a | b \ \ \ \ &:\ \ \ \ \txt{$a$ "given" (or such that) $b$.} \\
\mathcal{N}(u|\mu,\sigma^2)\ \ \ \ &:\ \ \ \ \txt{a Gaussian distribution for the random variable $u$}\\ 
&\ \ \ \ \ \ \ \txt{with mean $\mu$ and variance $\sigma^2$.}&\\
\delta(x)\ \ \ \ &:\ \ \ \ \txt{the delta Dirac function (which is formally a distribution)} \\ 
&\ \ \ \ \ \ \ \txt{that is a probability density giving a infinite weight to the single value $x=0$.} \\
\delta_{ij}\ \ \ \ &:\ \ \ \ \txt{the kronecker symbol, which is one if $i=j$, $0$ else.}\\
\partial i \defeq \{j:(ij)\in E\} \ \ \ \ &:\ \ \ \ \txt{the set of neighbors nodes to node $i$ in the}\\ 
&\ \ \ \ \ \ \ \txt{graphical representation of the problem ($E$ is the set of edges).}\\
\partial i\backslash j \ \ \ \ &:\ \ \ \ \txt{the set of neighbors nodes to node $i$ except the node $j$}\\ 
&\ \ \ \ \ \ \ \txt{in the graphical representation of the problem.}\\
u \sim P (u | \bsy{\theta})\ \ \ \ &:\ \ \ \ \txt{$u$ is a random variable with distribution $P(u | \bsy{\theta})$}\\ 
&\ \ \ \ \ \ \ \txt{that depends on a vector of parameters} \ \bsy{\theta}. \\
\mE_x(y(x))=\mE_P(y(x))\ \ \ \ &:\ \ \ \ \txt{the average of the function $y(x)$ with respect to the random}\\
&\ \ \ \ \ \ \ \txt{variable $x\sim P(x)$. The two notations are used equivalently}\\
&\ \ \ \ \ \ \ \txt{when there are no possible ambiguities.}\\
<\bx> \defeq 1/N\sum_i^N x_i\ \ \ \ &:\ \ \ \ \txt{the empirical average of the vector $\bx$ (here there are $N$ components).}\\
\big\{x_i | f(x_i)\big\}_{g(i)}^b\ \ \ \ &:\ \ \ \ \txt{the ensemble made of $\{x_i\}$ that verify the conditions}\\
&\ \ \ \ \ \ \ \txt{$f(x_i) \ \forall \ i\in \{1,...,b | g(i) \ \txt{is true}\}$.}\\
&\ \ \ \ \ \ \ \txt{As for any operations such as sums, products, etc,}\\
&\ \ \ \ \ \ \ \txt{if the lower bound of the index is not explicited, it means it starts from $1$.}\\
&\ \ \ \ \ \ \ \txt{For example, $\{a_i|a_i>0\}_i^N=\{a_i|a_i>0\}_{i=1}^N$, $\sum_{i}^N x_i=\sum_{i=1}^N x_i$, etc.}\\
\big[x_i | f(x_i)\big]_{g(i)}^b\ \ \ \ &:\ \ \ \ \txt{the concatenation of $\big\{x_i | f(x_i)\big\}_{g(i)}^b$ to form a vector}\\
&\ \ \ \ \ \ \ \txt{of cardinality that depends on $g$ and $b$.}\\
[a, b]\ \ \ \ &:\ \ \ \ \txt{the simple concatenation of $a$ and $b$ to form a vector.}\\
\mathbb{I}(E)\ \ \ \ &:\ \ \ \ \txt{the indicator function, which is $1$ if the condition $E$ is true, $0$ else.}\\
\Delta\ \ \ \ &:\ \ \ \ \txt{the variance of the i.i.d Gaussian measurement noise.} \\
\bsy \xi \defeq \big[\xi_\mu \sim \mathcal{N}(\xi_\mu|0,\Delta)\big]_\mu^M\ \ \ \ &:\ \ \ \ \txt{the i.i.d Gaussian measurement noise vector.} \\
||\tbf y||_p \defeq 1/M \bigg(\sum_i^M |y_i|^p\bigg)^{1/p}\ \ \ \ &:\ \ \ \ \txt{the rescaled $\ell_p$ norm of $\tbf y$, which is here of size} \ M.\\
\rm{snr} \defeq ||\tbf y||^2_2 / \Delta \ \ \ \ &:\ \ \ \ \txt{the signal to noise ratio, where $y$ is the codeword.}& \\
z \in O(u)\ \ \ \ &:\ \ \ \ z \ \txt{is a quantity of the same order as} \ u \ \txt{i.e.}\ z = Cu \\ & \ \ \ \ \ \ \ \txt{where $C$ is a constant that does not scale with the problem size $N$.}
\end{flalign*}
%
%
%
%
%
%
\begin{flalign*}
z \in o(u)\ \ \ \ &:\ \ \ \ z \ \txt{is a quantity at least an order smaller than} \ u \ \txt{i.e.} \lim \frac{z}{u} = 0 \\
&\ \ \ \ \ \ \ \txt{in a proper limit that depends on the context.}\\
a \approx b \ \ \ \ &:\ \ \ \ \txt{$a$ and $b$ are equal up to a negligible difference $\in o(a)$.} \\
\bx_{\backslash i}\defeq \big[x_j\big]_{j\neq i}^N\ \ \ \ &:\ \ \ \ \txt{the vector made of the $N-1$ components}\\
&\ \ \ \ \ \ \  \txt{of $\bx$ that are not the $i^{th}$ one.}\\
\bx_{a \backslash i}\defeq \big[x_j\in \partial a\big]_{j\neq i}\ \ \ \ &:\ \ \ \ \txt{the vector of components of $\bx$ that are neighbors}\\
&\ \ \ \ \ \ \  \txt{of the factor $a$, except the $i^{th}$ one.}\\
d\bx \defeq \prod_i^N dx_i\ \ \ \ &:\ \ \ \ \txt{integration over all the components of the size $N$ vector $\bx$.}& \\
\mathcal{D}\bx \defeq \prod_i^N \mathcal{D}x_i = \prod_i^N dx_i \mathcal{N}(x_i|0,1)\ \ \ \ &:\ \ \ \ \txt{integration over all the components of the size $N$ vector $\bx$}\\
&\ \ \ \ \ \ \  \txt{with unit centered Gaussian measure.} \\
\bX^{\intercal} \ \ \ \ &:\ \ \ \ \txt{the transpose of a vector or matrix.}\\
\bx^{a}\defeq \big[x_i^a\big]_i^N \ \ \ \ &:\ \ \ \ \txt{the component wise power operation for a vector (or matrix).}\\
\tbf X\tbf Y\defeq \tbf Z \ \txt{where $Z_{ij}=X_{ij}Y_{ij}$} \ \ \ \ &:\ \ \ \ \txt{the component wise product between matrices}\\
&\ \ \ \ \ \ \ \txt{or vectors of same size.}\\
\bx^{\intercal} \by = \bx \by^{\intercal} \defeq \sum_i^N x_iy_i \ \ \ \ &:\ \ \ \ \txt{the scalar product between two vectors of size $N$.}\\
&\ \ \ \ \ \ \ \txt{The two notations are equivalent as we always assume the}\\
&\ \ \ \ \ \ \ \txt{vectors to have proper dimensions to apply the product.}\\
\bF \bx \defeq \big[\sum_i^N F_{\mu i} x_i\big]_\mu^M\ \ \ \ &:\ \ \ \ \txt{the matrix product between $\bF$ of size $M\times N$ and $\bx$ of size $N$.}\\
(\bF \bx)_\mu \defeq\sum_i^N F_{\mu i} x_i\ \ \ \ &:\ \ \ \ \txt{the $\mu^{th}$ component of the vector $\bF \bx$.}\\
\txt{Var}_P(u)\defeq \mathbb{E}_P(u^2)-\mathbb{E}_P(u)^2\ \ \ \ &:\ \ \ \ \txt{the variance of the random variable $u$ with distribution $P$.}\\
\txt{inv}\(\bA\)\ \ \ \ &:\ \ \ \ \txt{the inverse of the matrix $A$.}\\
\partial_x \ \ \ &:\ \ \ \ \txt{the partial derivative with respect to $x$.}\\
|\bx| \ \ \ &:\ \ \ \ \txt{the number of components of $\bx$ or the cardinality of an ensemble.}\\
a\propto b \ \ \ &:\ \ \ \ \txt{$a$ is proportional to $b$, i.e. they are equal up to a constant.}
\end{flalign*}
%
%
%
%
%
%
\newpage
\begin{flalign*}
\txt{CS}\ \ \ \ &:\ \ \ \ \txt{compressed sensing.}&\\
\txt{MSE}\ \ \ \ &:\ \ \ \ \txt{mean squarre error.}\\
\txt{MMSE}\ \ \ \ &:\ \ \ \ \txt{minimum mean squarre error.}\\
\txt{MAP}\ \ \ \ &:\ \ \ \ \txt{maximum à posteriori.}\\
\txt{i.e.}\ \ \ \ &:\ \ \ \ \txt{id est.}\\
N\txt{-d}\ \ \ \ &:\ \ \ \ N\txt{-dimensional.}\\
\txt{BP}\ \ \ \ &:\ \ \ \ \txt{belief propagation.}\\
\txt{AMP}\ \ \ \ &:\ \ \ \ \txt{approximate message passing.}\\
\txt{SE}\ \ \ \ &:\ \ \ \ \txt{state evolution analysis.}\\
\txt{i.i.d}\ \ \ \ &:\ \ \ \ \txt{independent and identically distributed.}\\
\txt{AWGN}\ \ \ \ &:\ \ \ \ \txt{additive white Gaussian noise.} \\
\txt{EM}\ \ \ \ &:\ \ \ \ \txt{expectation maximization.}
\end{flalign*}
